Exploring the consequences of cyber attacks on Powertrain Cyber Physical Systems

This paper proposes a novel approach for the study of cyber-attacks against the powertrain of a generic vehicle. The proposed model is composed by a a generic Internal Combustion engine and a speed controller, that communicate through a Controller Area Network (CAN) bus. We consider a threat model composed by three representative attack scenarios designed to modify the output of the model, thus affecting the rotational speed of the engine. Two attack scenarios target both vehicle sensor systems and CAN communication, while one attack scenario only requires injection of CAN messages. To the best of our knowledge, this is the first attempt of modeling the consequences of realistic cyber attacks against a modern vehicle.

==> Makefile <==
TEX_FILES := $(wildcard *.tex)
TEX_FILES += $(wildcard sections/*.tex)
TEX_FILES += $(wildcard sections/appendix/*.tex)
TEX_FILES += $(wildcard tables/*.tex)
TEX_FILES += $(wildcard bio/*.tex)
BIB_FILES := $(wildcard sections/*.bib)
IMAGES_FILES += $(wildcard images/*)


all : main.pdf

main.pdf: main.aux $(TEX_FILES) $(IMAGES_FILES)
	pdflatex main.tex
	exiftool -Title="Exploring the consequences of cyber attacks on Powertrain Cyber Physical Systems" \
			 -Author="Stabili Romagnoli Marchetti Sinopoli Colajanni" main.pdf

main.aux: $(BIB_FILES)
	pdflatex main.tex
	bibtex main.aux
	pdflatex main.tex
	pdflatex main.tex

clean:
	rm main.pdf main.pdf_original *.aux *.blg *.log *.bbl || exit 0

